Boosting Fast Adversarial Training with Learnable Adversarial Initialization

Adversarial training (AT) has been demonstrated to be effective in improving model robustness by leveraging adversarial examples for training. However, most AT methods are in face of expensive time and computational cost for calculating gradients at multiple steps in generating adversarial examples. To boost training efficiency, fast gradient sign method (FGSM) is adopted in fast AT methods by calculating gradient only once. Unfortunately, the robustness is far from satisfactory. One reason may arise from the initialization fashion. Existing fast AT generally uses a random sample-agnostic initialization, which facilitates the efficiency yet hinders a further robustness improvement. Up to now, the initialization in fast AT is still not extensively explored. In this paper, we boost fast AT with a sample-dependent adversarial initialization, i.e., an output from a generative network conditioned on a benign image and its gradient information from the target network. As the generative network and the target network are optimized jointly in the training phase, the former can adaptively generate an effective initialization with respect to the latter, which motivates gradually improved robustness. Experimental evaluations on four benchmark databases demonstrate the superiority of our proposed method over state-of-the-art fast AT methods, as well as comparable robustness to advanced multi-step AT methods. The code is released at https://github.com//jiaxiaojunQAQ//FGSM-SDI.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> figtex/fig_step_size.tex <==
\begin{figure*}
\begin{center}
 \includegraphics[width=1\linewidth]{images/step_size.pdf}
\end{center}
\vspace{-6mm}
\caption{Accuracy of FGSM-SDI-AT and PGD-AT \cite{rice2020overfitting} on the adversarial examples generated by PGD-10 with different step sizes under $\epsilon =8$. }
\label{fig:step_size}
\end{figure*}

==> table/Ablation.tex <==
\begin{table*}[t]
\centering
\caption{Ablation study of the inputs of the generative network on the CIFAR10 database. Numbers in table represent percentage. Number in bold indicates the best.}
 \label{table:ablation}
 \scalebox{0.9}{
\begin{tabular}{c|ccccc|ccccc}
\toprule
\multicolumn{1}{c|}{Input} &       & Clean & PGD-10 & PGD-20 & PGD-50 & APGD  & APGD-T & FAB   & SQUARE & AA    \\ \hline
   \multirow{2}{*}{Benign}   & Best & 73.34 & 42.63  & 41.82  & 41.66  & 41.31 & 36.78  & 37.19 & 44.29  & 36.72 \\ %\cline{2-11} 
                            & Last & \textbf{89.64} & 21.34  & 13.72  & 7.59   & 4.04  & 0.00   & 0.00  & 11.97  & 0.00  \\ \hline
\multirow{2}{*}{Grad}       & Best & \textbf{86.08} & 50.09  & 48.44  & 47.97  & 47.49 & 44.29  & 44.89 & \textbf{55.64}  & 44.26 \\ %\cline{2-11} 
                            & Last & 86.08 & 50.09  & 48.44  & 47.97  & 47.49 & 44.29  & 44.89 & 55.64  & 44.26 \\ \hline
\multirow{2}{*}{Benign+Grad} & Best & 84.14 & \textbf{52.49}  & \textbf{51.37}  & \textbf{50.8}   & \textbf{50.24} & \textbf{47.26}  & \textbf{47.87} & {55.50}  & \textbf{47.28} \\ %\cline{2-11} 
                            & Last & 84.61 & \textbf{52.35}  & \textbf{51.02}  & \textbf{50.68}  & \textbf{50.14} & \textbf{46.79}  & \textbf{47.58} & \textbf{55.85}  & \textbf{46.78} \\ \bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}

==> table/Ablation_PGD_2.tex <==
\begin{table*}[t]
\centering
\caption{Comparisons with PGD2-AT on CIFAR10 database. Numbers in table represent percentage. Number in bold indicates the best. }
 \label{table:ablation_pdg_2}
 \scalebox{0.9}{
\begin{tabular}{c|ccccc|ccccc}
\toprule
Method                     &      & Clean          & PGD-10         & PGD-20         & PGD-50         & APGD           & APGD-T         & FAB            & SQUARE         & AA             \\ \hline
\multirow{2}{*}{PGD2-AT \cite{rice2020overfitting}} & Best & \textbf{89.93} & 39.50          & 37.26          & 36.47          & 35.99          & 34.88          & 35.84          & 51.73          & 34.84          \\ %\cline{2-11} 
                           & Last & \textbf{90.00} & 38.96          & 36.69          & 35.86          & 35.24          & 34.28          & 35.29          & 51.32          & 34.24          \\ \hline
\multirow{2}{*}{FGSM-SDI (Ours)}  & Best & 84.14          & \textbf{52.49} & \textbf{51.37} & \textbf{50.80} & \textbf{50.24} & \textbf{47.26} & \textbf{47.87} & \textbf{55.50} & \textbf{47.28} \\ %\cline{2-11} 
                           & Last & 84.61          & \textbf{52.35} & \textbf{51.02} & \textbf{50.68} & \textbf{50.14} & \textbf{46.79} & \textbf{47.58} & \textbf{55.85} & \textbf{46.78} \\ \bottomrule
\end{tabular}
}
\end{table*}

==> table/Imagenet.tex <==
\begin{table*}[t]
\centering
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) on the Tiny ImageNet database. Number in bold indicates the best of the fast AT methods. }
\label{table:Imagnet}
 \scalebox{0.9}{
\begin{tabular}{c|ccccc|ccccc|c}
\toprule
\multicolumn{1}{c|}{Method} &         & Clean & PGD-10 & PGD-20 & PGD-50 & APGD  & APGD-T & FAB   & SQUARE & AA    & Time(min)              \\ \hline
\multirow{2}{*}{PGD-AT \cite{rice2020overfitting}}       & Best & 43.60 & 20.20  & 19.90  & 19.86  & 19.64 & 16.00  & 16.26 & 21.98  & 16.00 & \multirow{2}{*}{1833} \\ %\cline{2-11}
                              & Last & 45.28 & 16.12  & 15.60  & 15.40  & 15.22 & 12.80  & 13.08 & 20.62  & 12.84 &                       \\ \hline \hline
\multirow{2}{*}{FGSM-RS \cite{wong2020fast}}   & Best & 44.98 & 17.72  & 17.46  & 17.36  & 17.22 & 14.12  & 14.3  & 21.52  & 14.08 & \multirow{2}{*}{339}  \\ %\cline{2-11}
                              & Last & 45.18 & 0.00   & 0.00   & 0.00   & 0.00  & 0.00   & 0.06  & 0.28   & 0.00  &                       \\ \hline
\multirow{2}{*}{FGSM-CKPT \cite{kim2020understanding}} & Best & \textbf{49.98} & 9.20   & 8.84   & 8.68   & 8.50  & 8.12   & 8.38  & 16.86  & 8.10  & \multirow{2}{*}{686}  \\ %\cline{2-11}
                              & Last & \textbf{49.98} & 9.20   & 8.84   & 8.68   & 8.50  & 8.12   & 8.38  & 16.86  & 8.10  &                       \\ \hline
\multirow{2}{*}{FGSM-GA \cite{andriushchenko2020understanding}}   & Best & 34.04 & 5.58   & 5.28   & 5.10   & 4.74  & 4.36   & 4.52  & 8.46   & 4.34  & \multirow{2}{*}{1054} \\ %\cline{2-11}
                              & Last & 34.04 & 5.58   & 5.28   & 5.10   & 4.74  & 4.36   & 4.52  & 8.46   & 4.34  &                       \\ \hline
\multirow{2}{*}{Free \cite{shafahi2019adversarial}}      & Best & 38.90 & 11.62  & 11.24  & 11.02  & 10.88 & 9.26   & 9.42  & 14.68  & 9.28  & \multirow{2}{*}{1375} \\ %\cline{2-11}
                              & Last & 40.06 & 8.84   & 8.32   & 8.20   & 7.94  & 7.36   & 7.60  & 12.16  & 7.34  &                       \\ \hline

\multirow{2}{*}{FGSM-SDI (Ours)}  & Best & 45.84 & \textbf{23.82}  & \textbf{23.30}  & \textbf{23.20}  & \textbf{22.44} & \textbf{15.82}  & \textbf{16.54} & \textbf{24.32}  & \textbf{15.78} & \multirow{2}{*}{926}  \\ %\cline{2-11}
                              & Last & 48.40  & \textbf{22.46}  & \textbf{21.08}  & \textbf{20.46}  & \textbf{17.16} & \textbf{11.14}  & \textbf{13.62} & \textbf{22.24}  & \textbf{11.10}&                       \\ \bottomrule
\end{tabular}
}
\end{table*}

==> table/Larger_ImageNet.tex <==
\begin{table}[]
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) with Resnet50 on the  ImageNet database. Number in bold indicates the best of the fast AT methods. }
\label{table:Larger_Imagnet}

\resizebox{\columnwidth}{!}{

\begin{tabular}{c|c|c|c|c|c}
\hline
ImageNet                         & Epsilon      & Clean  & PGD-10 & PGD-50 & Time(hour)             \\ \hline
\multirow{3}{*}{PGD-AT}          & $\epsilon=$2 & 64.39  & 47.536 & 47.502 & \multirow{3}{*}{211.2} \\ \cline{2-5}
                                 & $\epsilon=$4 & 58.668 & 35.730 & 35.216 &                        \\ \cline{2-5}
                                 & $\epsilon=$8 & 49.520 & 26.194 & 21.172 &                        \\ \hline\hline
\multirow{3}{*}{Free-AT(m=4)}    & $\epsilon=$2 & 68.37  & 48.31  & 48.28  & \multirow{3}{*}{127.7} \\ \cline{2-5}
                                 & $\epsilon=$4 & 63.42  & 33.22  & 33.08  &                        \\ \cline{2-5}
                                 & $\epsilon=$8 & 52.09  & 19.46  & 12.92  &                        \\ \hline
\multirow{3}{*}{FGSM-RS}         & $\epsilon=$2 & 67.65  & 48.78  & 48.67  & \multirow{3}{*}{44.5}  \\ \cline{2-5}
                                 & $\epsilon=$4 & 63.65  & 35.01  & 32.66  &                        \\ \cline{2-5}
                                 & $\epsilon=$8 & 53.89  & 0.00   & 0.00   &                        \\ \hline
\multirow{3}{*}{FGSM-SDI (ours)} & $\epsilon=$2 &     64.13   &    48.18    &    48.00    & \multirow{3}{*}{66.8}  \\ \cline{2-5}
                                 & $\epsilon=$4 &    57.81    &    36.16    &     35.40   &                        \\ \cline{2-5}
                                 & $\epsilon=$8 &   47.62     &   26.12     &   21.01     &                        \\ \hline
\end{tabular}
}
\vspace{-5mm}
\end{table}

==> table/Selection.tex <==
\begin{table*}[t]
\caption{The hyperparameter selection on the CIFAR10 database. Numbers in table represent percentage. Number in bold indicates the best }
\centering
\label{table:selection}
 \scalebox{1.0}{
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
     & Clean                  & PGD-10         & PGD-20         & PGD-50         & C\&W      & APGD      & AA             & Time(min)   \\ \hline
k=1  & \textbf{85.05}           & 52.95          & 51.52          & 51.16          & 49.80     & 50.64    & 47.06          & 134         \\ \hline
k=2  & 85.14                   & 52.63          & 51.26          & 50.9           & 49.75     & 50.42    & 47.36          & 106         \\ \hline
k=10 & 84.80                    & 53.33          & 52.20          & 51.79          & 50.47    &  51.52    & 47.99          & 84          \\ \hline
k=20 & 84.86           & \textbf{53.73} & \textbf{52.54} & \textbf{52.18} & \textbf{51.00} & \textbf{51.84} & \textbf{48.52} & 83 \\ \hline
k=30 & 84.45                 & 53.30          & 52.09          & 51.77          & 50.09   &   51.05     & 47.03          & 82          \\ \hline
k=40 & 84.73                    & 52.96          & 51.71          & 51.34          & 49.62     & 51.01    & 47.24          & \textbf{81}         \\ \hline
\end{tabular}
}
\end{table*}

==> table/cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) on the CIFAR10 database. Number in bold indicates the best of the fast AT methods. }
\label{table:cifar10}
 \scalebox{0.9}{
\begin{tabular}{c|ccccc|ccccc|c}
\toprule
\multicolumn{1}{c|}{Method} &        & Clean & PGD-10 & PGD-20 & PGD-50 & APGD  & APGD-T & FAB   & SQUARE & AA    & \multicolumn{1}{l}{Time(min)} \\ \hline
\multirow{2}{*}{PGD-AT \cite{rice2020overfitting}}       & Best & 82.64 & 53.15  & 52.56  & 52.15  & 52.02 & 48.81  & 49.27 & 56.31  & 48.81 & \multirow{2}{*}{261}          \\ %\cline{2-11}
                              & Last & 82.86 & 52.85  & 52.27  & 51.98  & 51.72 & 48.52  & 48.91 & 56.07  & 48.54 &                               \\ \hline\hline
\multirow{2}{*}{FGSM-RS \cite{wong2020fast}}   & Best & 73.81 & 42.31  & 41.55  & 41.26  & 41.02 & 37.04  & 37.42 & 45.44  & 37.07 & \multirow{2}{*}{55}           \\ %\cline{2-11}
                              & Last & 83.82 & 0.09   & 0.04   & 0.02   & 0.02  & 0.00   & 0.00  & 0.00   & 0.00  &                               \\ \hline
\multirow{2}{*}{FGSM-CKPT \cite{kim2020understanding}} & Best & \textbf{88.29} & 42.05  & 39.8   & 39.11  & 38.45 & 37.27  & 38.23 & 52.80  & 37.15 & \multirow{2}{*}{83}           \\ %\cline{2-11}
                              & Last & \textbf{88.29} & 42.05  & 39.8   & 39.11  & 38.45 & 37.27  & 38.23 & 52.80  & 37.15 &                               \\ \hline
\multirow{2}{*}{FGSM-GA \cite{andriushchenko2020understanding}}   & Best & 83.96 & 49.23  & 47.57  & 46.89  & 45.86 & 43.46  & 44.52 & 53.83  & 43.45 & \multirow{2}{*}{193}          \\ %\cline{2-11}
                              & Last & 84.43 & 48.67  & 46.66  & 46.08  & 45.05 & 42.75  & 43.71 & 53.76  & 42.63 &                               \\ \hline
\multirow{2}{*}{Free \cite{shafahi2019adversarial}}      & Best & 74.87 & 43.58  & 42.81  & 42.62  & 42.38 & 39.07  & 39.57 & 46.21  & 39.05 & \multirow{2}{*}{215}          \\ %\cline{2-11}
                              & Last & 74.87 & 43.7   & 42.84  & 42.6   & 42.34 & 39.11  & 39.59 & 46.31  & 39.11 &                               \\ \hline
\multirow{2}{*}{FGSM-SDI (Ours)}  & Best & 84.14 & \textbf{52.49}  & \textbf{ 51.37}  &  \textbf{50.8}   &  \textbf{50.24} &  \textbf{47.26}  &  \textbf{47.87} &  \textbf{55.50}  &  \textbf{47.28} & \multirow{2}{*}{137}          \\ %\cline{2-11}
                              & Last & 84.61 &  \textbf{52.35}  &  \textbf{51.02}  &  \textbf{50.68}  &  \textbf{50.14} &  \textbf{46.79}  &  \textbf{47.58} &  \textbf{55.85}  &  \textbf{46.78} &                               \\ \bottomrule
\end{tabular}
}
\end{table*}

==> table/cifar100.tex <==
\begin{table*}[t]
\centering
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) on the CIFAR100 database. Number in bold indicates the best of the fast AT methods. }
\label{table:cifar100}
 \scalebox{0.9}{
\begin{tabular}{c|ccccc|ccccc|c}
\toprule
\multicolumn{1}{c|}{Method}    &     & Clean & PGD-10 & PGD-20 & PGD-50 & APGD  & APGD-T & FAB   & SQUARE & AA    & Time(min)             \\ \hline
\multirow{2}{*}{PGD-AT \cite{rice2020overfitting}}       & Best & 57.52 & 29.60  & 28.99  & 28.87  & 28.60 & 25.50  & 25.80 & 30.58  & 25.48 & \multirow{2}{*}{284} \\ %\cline{2-11}
                              & Last & 57.50 & 29.54  & 29.00  & 28.90  & 28.70 & 25.51  & 25.78 & 30.58  & 25.48 &                      \\ \hline\hline
\multirow{2}{*}{FGSM-RS \cite{wong2020fast}}   & Best & 49.85 & 22.47  & 22.01  & 21.82  & 21.62 & 18.32  & 18.56 & 23.26  & 18.29 & \multirow{2}{*}{70}  \\ %\cline{2-11}
                              & Last & 60.55 & 0.45   & 0.25   & 0.19   & 0.00  & 0.00   & 0.02  & 3.52   & 0.00  &                      \\ \hline
\multirow{2}{*}{FGSM-CKPT \cite{kim2020understanding}} & Best & \textbf{60.93} & 16.58  & 15.47  & 15.19  & 14.63 & 14.27  & 14.72 & 21.53  & 14.17 & \multirow{2}{*}{92}  \\ %\cline{2-11}
                              & Last & \textbf{60.93} & 16.69  & 15.61  & 15.24  & 14.87 & 14.42  & 14.80 & 21.38  & 14.34 &                      \\ \hline
\multirow{2}{*}{FGSM-GA \cite{andriushchenko2020understanding}}   & Best & 47.57 & 21.33  & 20.83  & 20.64  & 20.37 & 17.20  & 17.4  & 21.70  & 17.2  & \multirow{2}{*}{202} \\ %\cline{2-11}
                              & Last & 55.1  & 18.84  & 17.95  & 17.72  & 17.41 & 16.14  & 16.39 & 21.32  & 16.1  &                      \\ \hline

\multirow{2}{*}{Free \cite{goodfellow2014explaining}}      & Best & 44.03 & 20.61  & 20.23  & 20.23  & 19.98 & 16.47  & 16.65 & 20.19  & 16.46 & \multirow{2}{*}{229} \\ %\cline{2-11}
                              & Last & 48.03 & 20.17  & 20.29  & 20.19  & 20.00 & 16.47  & 16.64 & 20.22  & 16.46 &                      \\ \hline

\multirow{2}{*}{FGSM-SDI (Ours)}  & Best & 59.76 & \textbf{31.46}  & \textbf{30.81}  & \textbf{30.52}  & \textbf{29.66 }& \textbf{25.08 } & \textbf{25.81} & \textbf{31.01}  & \textbf{25.09} & \multirow{2}{*}{154} \\ %\cline{2-11}
                              & Last & 59.99 & \textbf{31.34}  & \textbf{30.47}  & \textbf{30.29}  & \textbf{29.39} & \textbf{24.63}  & \textbf{25.36} & \textbf{30.87}  & \textbf{24.63} &                      \\ \bottomrule
\end{tabular}
}
\end{table*}

==> table/cifar100_v2.tex <==
\begin{table*}[t]
\centering
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) with Resnet18 on the CIFAR100 database. Number in bold indicates the best of the fast AT methods. }
\label{table:cifar100}
 \scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
Target Network             & Method                          &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W             & APGD           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{Resnet18}  & \multirow{2}{*}{PGD-AT}         & Best & 57.52          & 29.6           & 28.99          & 28.87          & 28.85          & 28.60          & 25.48          & \multirow{2}{*}{284} \\ \cline{3-10}
                           &                                 & Last & 57.5           & 29.54          & 29.00          & 28.90          & 27.6           & 28.70          & 25.48          &                      \\ \hline \hline
\multirow{10}{*}{Resnet18} & \multirow{2}{*}{FGSM-RS}        & Best & 49.85          & 22.47          & 22.01          & 21.82          & 20.55          & 21.62          & 18.29          & \multirow{2}{*}{70}  \\ \cline{3-10}
                           &                                 & Last & 60.55          & 00.45          & 00.25          & 00.19          & 00.25          & 0.00           & 0.00           &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-CKPT}      & Best & \textbf{60.93} & 16.58          & 15.47          & 15.19          & 16.4           & 14.63          & 14.17          & \multirow{2}{*}{96}  \\ \cline{3-10}
                           &                                 & Last & \textbf{60.93} & 16.69          & 15.61          & 15.24          & 16.6           & 14.87          & 14.34          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-GA}        & Best & 54.35          & 22.93          & 22.36           & 22.2         & 21.2          & 21.88          &     18.88      & \multirow{2}{*}{187} \\ \cline{3-10}
                           &                                 & Last & 55.1           & 20.04          & 19.13          & 18.84          & 18.96          & 18.46          & 16.45          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{Free-AT(m=8)}   & Best & 44.03          & 20.61          & 20.23          & 20.23          & 18.26          & 19.98          & 16.46          & \multirow{2}{*}{229} \\ \cline{3-10}
                           &                                 & Last & 48.03          & 20.17          & 20.29          & 20.19          & 18.20          & 20.00          & 16.46          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-SDI(ours)} & Best & 60.67          & \textbf{31.5}  & \textbf{30.89} & \textbf{30.6}  & \textbf{27.15} & \textbf{30.26} & \textbf{25.23} & \multirow{2}{*}{99}  \\ \cline{3-10}
                           &                                 & Last & 60.82          & \textbf{30.87} & \textbf{30.34} & \textbf{30.08} & \textbf{27.3}  & \textbf{29.94} & \textbf{25.19} &                      \\ \hline
\end{tabular}
}
\end{table*}

==> table/cifar100_v3.tex <==
\begin{table*}[t]
\centering
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) with Resnet18 on the CIFAR100 database. Number in bold indicates the best of the fast AT methods. }
\label{table:cifar100}
 \scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
Target Network             & Method                          &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W             & APGD           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{Resnet18}  & \multirow{2}{*}{PGD-AT}         & Best & 57.52          & 29.6           & 28.99          & 28.87          & 28.85          & 28.60          & 25.48          & \multirow{2}{*}{284} \\ \cline{3-10}
                           &                                 & Last & 57.5           & 29.54          & 29.00          & 28.90          & 27.6           & 28.70          & 25.48          &                      \\ \hline \hline
\multirow{10}{*}{Resnet18} & \multirow{2}{*}{FGSM-RS}        & Best & 49.85          & 22.47          & 22.01          & 21.82          & 20.55          & 21.62          & 18.29          & \multirow{2}{*}{70}  \\ \cline{3-10}
                           &                                 & Last & 60.55          & 00.45          & 00.25          & 00.19          & 00.25          & 0.00           & 0.00           &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-CKPT}      & Best & \textbf{60.93} & 16.58          & 15.47          & 15.19          & 16.4           & 14.63          & 14.17          & \multirow{2}{*}{96}  \\ \cline{3-10}
                           &                                 & Last & \textbf{60.93} & 16.69          & 15.61          & 15.24          & 16.6           & 14.87          & 14.34          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-GA}        & Best & 54.35          & 22.93          & 22.36           & 22.2         & 21.2          & 21.88          &     18.88      & \multirow{2}{*}{187} \\ \cline{3-10}
                           &                                 & Last & 55.1           & 20.04          & 19.13          & 18.84          & 18.96          & 18.46          & 16.45          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{Free-AT(m=8)}   & Best & 57.37          & 25.81          & 25.12         & 24.89          & 23.92          & 24.56          & 21.88         & \multirow{2}{*}{229} \\ \cline{3-10}
                           &                                 & Last & 58.23          & 25.71          & 24.88          & 24.57          & 24.34          &  24.29          & 22.46          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-SDI(ours)} & Best & 60.67          & \textbf{31.5}  & \textbf{30.89} & \textbf{30.6}  & \textbf{27.15} & \textbf{30.26} & \textbf{25.23} & \multirow{2}{*}{99}  \\ \cline{3-10}
                           &                                 & Last & 60.82          & \textbf{30.87} & \textbf{30.34} & \textbf{30.08} & \textbf{27.3}  & \textbf{29.94} & \textbf{25.19} &                      \\ \hline
\end{tabular}
}
\end{table*}

==> table/cifar10_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) with Resnet18 on the CIFAR10 database. Number in bold indicates the best of the fast AT methods. }
\centering
\label{table:cifar10}
 \scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
Target Network             & Method                          &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W             & APGD           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{Resnet18}  & \multirow{2}{*}{PGD-AT}         & Best & 82.64          & 53.15          & 52.56          & 52.15          & 51.14          & 52.02          & 48.81          & \multirow{2}{*}{265} \\ \cline{3-10}
                           &                                 & Last & 82.86          & 52.85          & 52.27          & 51.98          & 51.32          & 51.72          & 48.54          &                      \\ \hline \hline
\multirow{10}{*}{Resnet18} & \multirow{2}{*}{FGSM-RS}        & Best & 73.81          & 42.31          & 41.55          & 41.26          & 39.84          & 41.02          & 37.07          & \multirow{2}{*}{51}  \\ \cline{3-10}
                           &                                 & Last & 83.82          & 00.09          & 00.04          & 00.02          & 0.00           & 0.00           & 0.00           &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-CKPT}      & Best & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 38.45          & 37.15          & \multirow{2}{*}{76}  \\ \cline{3-10}
                           &                                 & Last & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 38.45          & 37.15          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-GA}        & Best & 83.96          & 49.23          & 47.57          & 46.89          & 47.46          & 45.86          & 43.45          & \multirow{2}{*}{178} \\ \cline{3-10}
                           &                                 & Last & 84.43          & 48.67          & 46.66          & 46.08          & 46.75          & 45.05          & 42.63          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{Free-AT(m=8)}   & Best & 74.87          & 43.7           & 42.84          & 42.6           & 41.09          & 42.38          & 39.11          & \multirow{2}{*}{215} \\ \cline{3-10}
                           &                                 & Last & 74.87          & 43.58          & 42.81          & 42.62          & 41.1           & 42.34          & 39.05          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-SDI(ours)} & Best & 84.86          & \textbf{53.73} & \textbf{52.54} & \textbf{52.18} & \textbf{51.00} & \textbf{51.84} & \textbf{48.52} & \multirow{2}{*}{83}  \\ \cline{3-10}
                           &                                 & Last & 85.25          & \textbf{53.18} & \textbf{52.05} & \textbf{51.79} & \textbf{50.29} & \textbf{51.30} & \textbf{47.91} &                      \\ \hline
\end{tabular}
}
\end{table*}

==> table/cifar10_v3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) with Resnet18 on the CIFAR10 database. Number in bold indicates the best of the fast AT methods. }
\centering
\label{table:cifar10}
 \scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
Target Network             & Method                          &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W             & APGD           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{Resnet18}  & \multirow{2}{*}{PGD-AT}         & Best & 82.64          & 53.15          & 52.56          & 52.15          & 51.14          & 52.02          & 48.81          & \multirow{2}{*}{265} \\ \cline{3-10}
                           &                                 & Last & 82.86          & 52.85          & 52.27          & 51.98          & 51.32          & 51.72          & 48.54          &                      \\ \hline \hline
\multirow{10}{*}{Resnet18} & \multirow{2}{*}{FGSM-RS}        & Best & 73.81          & 42.31          & 41.55          & 41.26          & 39.84          & 41.02          & 37.07          & \multirow{2}{*}{51}  \\ \cline{3-10}
                           &                                 & Last & 83.82          & 00.09          & 00.04          & 00.02          & 0.00           & 0.00           & 0.00           &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-CKPT}      & Best & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 38.45          & 37.15          & \multirow{2}{*}{76}  \\ \cline{3-10}
                           &                                 & Last & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 38.45          & 37.15          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-GA}        & Best & 83.96          & 49.23          & 47.57          & 46.89          & 47.46          & 45.86          & 43.45          & \multirow{2}{*}{178} \\ \cline{3-10}
                           &                                 & Last & 84.43          & 48.67          & 46.66          & 46.08          & 46.75          & 45.05          & 42.63          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{Free-AT(m=8)}   & Best & 84.25          & 50.02           & 49.64          & 49.28           & 49.23          & 48.9          & 45.6          & \multirow{2}{*}{215} \\ \cline{3-10}
                           &                                 & Last & 84.86          & 49.76          & 49.6         & 49.21          & 49.3          & 48.89          & 45.51          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-SDI(ours)} & Best & 84.86          & \textbf{53.73} & \textbf{52.54} & \textbf{52.18} & \textbf{51.00} & \textbf{51.84} & \textbf{48.52} & \multirow{2}{*}{83}  \\ \cline{3-10}
                           &                                 & Last & 85.25          & \textbf{53.18} & \textbf{52.05} & \textbf{51.79} & \textbf{50.29} & \textbf{51.30} & \textbf{47.91} &                      \\ \hline
\end{tabular}
}
\end{table*}

==> table/cifar10_v4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) with Resnet18 on the CIFAR10 database. Number in bold indicates the best of the fast AT methods. }
\centering
\label{table:cifar10}
 \scalebox{0.9}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
Target Network             & Method                          &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W             & APGD           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{Resnet18}  & \multirow{2}{*}{PGD-AT}         & Best & 82.64          & 53.15          & 52.56          & 52.15          & 51.14          & 52.02          & 48.81          & \multirow{2}{*}{265} \\ \cline{3-10}
                           &                                 & Last & 82.86          & 52.85          & 52.27          & 51.98          & 51.32          & 51.72          & 48.54          &                      \\ \hline \hline
\multirow{10}{*}{Resnet18} & \multirow{2}{*}{FGSM-RS}        & Best & 73.81          & 42.31          & 41.55          & 41.26          & 39.84          & 41.02          & 37.07          & \multirow{2}{*}{51}  \\ \cline{3-10}
                           &                                 & Last & 83.82          & 00.09          & 00.04          & 00.02          & 0.00           & 0.00           & 0.00           &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-CKPT}      & Best & \textbf{90.29} & 42.05          & 39.80          & 39.11          & 41.46          & 38.45          & 37.15          & \multirow{2}{*}{76}  \\ \cline{3-10}
                           &                                 & Last & \textbf{90.29} & 42.05          & 39.80          & 39.11          & 41.46          & 38.45          & 37.15          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-GA}        & Best & 83.96          & 49.23          & 47.57          & 46.89          & 47.46          & 45.86          & 43.45          & \multirow{2}{*}{178} \\ \cline{3-10}
                           &                                 & Last & 84.43          & 48.67          & 46.66          & 46.08          & 46.75          & 45.05          & 42.63          &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{Free-AT(m=8)}   & Best & 80.38          & 47.1           & 45.85          & 45.62           & 44.42          & 42.18          & 42.17          & \multirow{2}{*}{215} \\ \cline{3-10}
                           &                                 & Last & 80.75          & 45.82          & 44.82         & 44.48          & 43.73          & 45.22          & 41.17         &                      \\ \cline{2-11} 
                           & \multirow{2}{*}{FGSM-SDI(ours)} & Best & 84.86          & \textbf{53.73} & \textbf{52.54} & \textbf{52.18} & \textbf{51.00} & \textbf{51.84} & \textbf{48.50} & \multirow{2}{*}{83}  \\ \cline{3-10}
                           &                                 & Last & 85.25          & \textbf{53.18} & \textbf{52.05} & \textbf{51.79} & \textbf{50.29} & \textbf{51.30} & \textbf{47.91} &                      \\ \hline
\end{tabular}
}
\end{table*}

==> table/cifar10_wide.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) with WideResNet34-10 on the CIFAR10 database. Number in bold indicates the best of the fast AT methods. }
\centering
\label{table:cifar10_wide}
 \scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
Target Network                    & Method                          &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & APGD           & AA             & Time(min)             \\ \hline
\multirow{2}{*}{WideResNet34-10}  & \multirow{2}{*}{PGD-AT}         & Best & 85.17          & 56.1           & 55.07          & 54.87          & 53.84          & 54.15          & 51.67          & \multirow{2}{*}{1914} \\ \cline{3-10}
                                  &                                 & Last & 86.98          & 53.16          & 51.92          & 51.65          & 52.42          & 51.25          & 49.81          &                       \\ \hline\hline
\multirow{10}{*}{WideResNet34-10} & \multirow{2}{*}{FGSM-RS}        & Best & 74.29          & 41.24          & 40.21          & 39.98          & 39.27          & 39.79          & 36.40          & \multirow{2}{*}{348}  \\ \cline{3-10}
                                  &                                 & Last & 80.83          & 0.00           & 0.00           & 0.00           & 0.00           & 0.00           & 0.00           &                       \\ \cline{2-11} 
                                  & \multirow{2}{*}{FGSM-CKPT}      & Best & \textbf{91.84} & 44.7           & 42.72          & 42.22          & 42.25          & 41.69          & 40.46          & \multirow{2}{*}{470}  \\ \cline{3-10}
                                  &                                 & Last & \textbf{91.84} & 44.7           & 42.72          & 42.22          & 42.25          & 41.69          & 40.46          &                       \\ \cline{2-11} 
                                  & \multirow{2}{*}{FGSM-GA}        & Best & 81.8           & 48.2           & 47.97          & 46.6           & 46.87          & 46.27          & 45.19          & \multirow{2}{*}{1218} \\ \cline{3-10}
                                  &                                 & Last & 86.45          & 47.57          & 46.3           & 45.65          & 45.32          & 45.20          & 44.10          &                       \\ \cline{2-11} 
                                  & \multirow{2}{*}{Free-AT(m=8)}   & Best & 81.15          & 47.46          & 46.82          & 46.68          & 44.93          & 47.34          & 43.94          & \multirow{2}{*}{1422} \\ \cline{3-10}
                                  &                                 & Last & 82.4           & 47.3           & 46.61          & 46.42          & 44.73          & 47.17          & 43.68          &                       \\ \cline{2-11} 
                                  & \multirow{2}{*}{FGSM-SDI(ours)} & Best & 86.4           & \textbf{55.89} & \textbf{54.95} & \textbf{54.6}  & \textbf{53.68} & \textbf{54.21} & \textbf{51.17} & \multirow{2}{*}{533}  \\ \cline{3-10}
                                  &                                 & Last & 87.71          & \textbf{54.73} & \textbf{52.8}  & \textbf{52.21} & \textbf{52.78} & \textbf{51.60} & \textbf{49.48} &                       \\ \hline
\end{tabular}
}
\end{table*}

==> tex/broader_impact.tex <==
\section*{Broader Impact}
AT is one of the most effective methods to improve the model robustness, but its high computational cost makes it difficult to be widely used in deep learning tasks. Although some fast AT methods reduce the computational cost, there is a big gap between their performance and multi-step AT. 

In this paper, we propose a novel fast AT method from the perspective of initialization. The proposed fast AT not only reduces the computational cost but also achieves comparable robustness to advanced multi-step AT methods which the previous fast AT methods have not achieved. It is worth mentioning that the proposed method only takes half the training time of advanced multi-step AT but achieves the same performance as advanced multi-step AT, which reduce the gap to advanced multi-step AT.

==> tex/checklist.tex <==

\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Our main contribution was clarified in introduction and abstract sections.}
  \item Did you describe the limitations of your work?
    \answerYes{The limitations were given in the conclusion section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The societal impacts are stated in Sec.~\ref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have read the ethics review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We did not include any theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We did not include any theoretical results.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We included them in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{They were clearly specified.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We run for 5 times in Appendix Table \ref{table:cifar10}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{They were given in Sec. \ref{sec:Experiments Setting}. One single NVIDIA Tesla V100 was used.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited their papers and provided their links.}
  \item Did you mention the license of the assets?
    \answerYes{We cited their papers and provided their links.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{ We did not include any new assets.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{CIFAR-10/100 and TinyImagenet are widely used directly in classification tasks. We conduct experiments on these open sourced data sets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{CIFAR-10/100 and TinyImagenet do not contain personally identifiable information or offensive content. }
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
\end{enumerate}

\end{enumerate}

\newpage
\appendix


==> tex/preliminary.tex <==
\section{Preliminary}
Adversarial training (AT) can be formulated as a min-max optimization problem,  i.e. the inner maximization maximizes the classification loss to generate adversarial examples and the outer minimization minimizes the loss on generated adversarial examples to train parameters of a robust model. Given a target network $f(\cdot, \mathbf{w})$ with parameters $\mathbf{w}$, a data distribution $\mathcal{D}$ including the benign sample $x$ and its corresponding label $y$, a loss function $\mathcal{L}(f(x, \mathbf{w}), y)$ and a threat bound $\triangle$.
The objective function of AT can be defined as:
\begin{equation}
\min_{\mathbf{w}} \mathbb{E}_{(x, y) \sim \mathcal{D}}\left[\max _{\delta \in \triangle} \mathcal{L}(f(x + \delta; \mathbf{w}), y)\right], \label{Eq:sat}
\end{equation}
where the threat bound can be defined as 
$\triangle=\{ \delta: \|\delta\| \leq \epsilon \}$ with the maximum perturbation intensity $\epsilon$. 
%The goal of inner maximization is to find an optimal perturbation $\delta$ to maximize the loss function and the goal of outer minimization is to find the an optimal robust parameter $\mathbf{w}$ to minimize the loss function on the generated adversarial example $x+\delta$. 
The core of the adversarial training is how to find a better adversarial perturbation $\delta$. 

On the one hand, typical adversarial training methods usually adopt a multi-step adversarial attack to generate adversarial perturbations $\delta$, i.e. multiple steps of projected gradient ascent (PGD) \cite{madry2017towards}. It can be defined as: 
 \begin{equation}
 \delta_{t+1} =\Pi_{[-\epsilon, \epsilon]^{d}} [ \delta_{t}+ \alpha \text{sign}(\nabla_{x}\mathcal{L}(f(x + \delta_{t}; \mathbf{w}), y) ) ],
 \end{equation}
 where $\Pi_{[-\epsilon, \epsilon]^{d}}$
 represents the the projection to $[-\epsilon, \epsilon]^{d}$ and $\delta_{t+1}$ represents adversarial perturbation after $t+1$ iteration steps.
 In general, more iterations can boost robustness in adversarial training due to generating stronger adversarial examples. The prime PGD-based adversarial training framework is proposed in \cite{madry2017towards}. Following this framework, a lager number of PGD-based AT methods are proposed, amongst which an early stopping version \cite{rice2020overfitting} outperforms. %which obtains a great improvement of the model robustness. 
 %However, PGD-based AT methods require a high computational cost to perform PGD attack. 
 The algorithm of PGD-AT variants is summarized in Algorithm \ref{alg:PGD_AT}. 
 
 %Thus, how to reduce the computational cost and accelerate adversarial training is an important research field for adversarial training. To achieve the efficiency of AT, in an extreme case,
 On the other hand, Fast AT variants are proposed by adopting Fast Gradient Sign Method (FGSM)   \cite{goodfellow2014explaining}, which is one-step PGD.
 %, is performed to generate adversarial examples. 
 It can be defined as:
  \begin{equation}
 \delta^{*} =\epsilon \text{sign}(\nabla_{x}\mathcal{L}(f(x; \mathbf{w}), y) ) ,
 \end{equation}
 where $\epsilon$ represents the maximal perturbation strength. This kind of adversarial  training can be called as FGSM-based AT. Although it 
 accelerates adversarial training, it severely damages the robustness of the model, i.e. it can not defend against the PGD attack. 
 In detail, FGSM-based AT has a catastrophic overfitting issue, i.e., the target model suddenly loses the robustness 
 accuracy of adversarial examples generated by PGD (on the training data) during training.
 Fortunately, in \cite{wong2020fast}, Wong \emph{et al}. propose using FGSM-based AT combined with a random initialization to relieve the catastrophic overfitting. And it
 can achieve the same performance as prime PGD-based AT \cite{madry2017towards}. In detail, they perform FGSM with a  random initialization $\eta \in \mathbf{U}(-\epsilon ,\epsilon)$, where $\mathbf{U}$ represents a uniform distribution, which can be called FGSM-RS-AT.
 It can be defined as:
 \begin{equation}
 \delta^{*} =\Pi_{[-\epsilon, \epsilon]^{d}} [ \eta+ \alpha \text{sign}(\nabla_{x}\mathcal{L}(f(x +\eta; \mathbf{w}), y) ) ],
 \end{equation}
 where $\alpha$ represents step size, which is set to $1.25\epsilon$ in \cite{wong2020fast}. This work demonstrates that combined with an good initialization, FGSM-based AT can achieve excellent performance as PGD-AT \cite{madry2017towards}. But compared with PGD-AT, the FGSM-RS-AT requires a lower computational cost. The FGSM-RS-AT algorithm is summarized in Algorithm \ref{alg:FGSM_AT}
 Moreover, following FGSM-RS-AT, several works are proposed to improve the model robustness. In \cite{andriushchenko2020understanding}, Andriushchenko \emph{et al}. find using a random initialization does not completely solve the catastrophic overfitting problem and propose a regularization method for FGSM-RS-AT, dubbed FGSM-GA-AT, to improve the performance of FGSM-based AT. Moreover, in \cite{kim2020understanding}, Kim \emph{et al}. propose a stable single-step adversarial training based on FGSM-RS-AT, which can be call FGSM-CKPT-AT.
 
 \input{algo/PGD_AT}
 \input{algo/FGSM_AT}

==> tex/related.tex <==
\section{Related Work}
In this section, we first introduce the related researches on the attack methods to generate adversarial examples. Then we introduce the related researches on the defense methods, especially the adversarial training variants. In this paper, we focus on the image classification task.
\subsection{Attack Methods}
Adversarial attacks can be divided into black-box attacks \cite{papernot2017practical} and white-box attacks \cite{goodfellow2014explaining}.

\subsection{Adversarial Training Methods}
Adversarial training (AT) variants have been widely accepted to improve adversarial robustness under comprehensively evaluations.
%against vast attack methods, \textit{e.g.}, gradient-based attack, optimization-based attack, etc.
Typical adversarial training methods adopt multi-step attack methods (\textit{e.g.}, iterative projected gradient descent, PGD) to generate adversarial examples in the training phase, causing a high computational and time cost.
Then a series of fast adversarial training methods are proposed to accelerate the training efficiency. 
%However, their robustness is much worse than multi-step ones.

\noindent
\textbf{Fast Adversarial Training.}
Free-AT \cite{shafahi2019adversarial} proposes to recycle the gradient information when model is updated to reduce the cost of adversarial examples generation.
FGSM-RS-AT \cite{wong2020fast}  proposes to adopt FGSM combined with a random initialization to conduct adversarial training. %although it achieves an exciting efficiency improvement, the adversarial accuracy especially against non-FGSM-series attack decreases a lot compared to PGD-based AT methods.
It eliminates the overhead cost of generating adversarial examples by using one simultaneous backward propagation for updating both the model parameters and image perturbations.
%recycling the gradient information computed when updating model parameters.
%FGSM\_RS updates both the model parameters and image perturbations using one simultaneous backward pass, rather than using separate gradient computations for each update step.
FGSM-CKPT-AT \cite{kim2020understanding} determines the appropriate magnitude of the perturbation for each image, and thus prevents catastrophic overfitting.
FGSM-GA-AT \cite{andriushchenko2020understanding} maximizes the gradient alignment inside the perturbation bound and therefore improves the quality of FGSM solution.
YOPO \cite{} observes that adversarial perturbation is only coupled with the first layer of neural networks, thus proposes to split the adversary computation and weight updating. Its adversarial computation is focused on the first layer.


\noindent
\textbf{Comprehensive Evaluations}
To conduct a comprehensive robustness evaluation, we briefly introduce and list adversarial attack methods used in our experiments, which strictly follow the updated evaluation strategy.
For white-box attack, we adopt PGD and FGSM, and CW. For adaptive attack, we adopt AutoAttack, which is composed of 4 adaptive attack methods including white-box and black-box ones.

As mentioned, existing Fast AT methods are now in face of poor robustness especially against stronger attacks. Although they achieve an exciting efficiency improvement, the adversarial accuracy especially against non-FGSM-series attack decreases a lot compared to multi-step PGD-based AT methods. One reason might be that they simply adopt the sample-agnostic initialization.
Therefore, we explore and optimize the adversarial initialization in fast-AT in the paper.
